Learning Stabilizing Controllers for Unstable Linear Quadratic Regulators from a Single Trajectory

The principal task to control dynamical systems is to ensure their stability. When the system is unknown, robust approaches are promising since they aim to stabilize a large set of plausible systems simultaneously. We study linear controllers under quadratic costs model also known as linear quadratic regulators (LQR). We present two different semi-definite programs (SDP) which results in a controller that stabilizes all systems within an ellipsoid uncertainty set. We further show that the feasibility conditions of the proposed SDPs are \emph{equivalent}. Using the derived robust controller syntheses, we propose an efficient data dependent algorithm -- \textsc{eXploration} -- that with high probability quickly identifies a stabilizing controller. Our approach can be used to initialize existing algorithms that require a stabilizing controller as an input while adding constant to the regret. We further propose different heuristics which empirically reduce the number of steps taken by \textsc{eXploration} and reduce the suffered cost while searching for a stabilizing controller.

==> bayesian_bounds_and_robust_formulations.tex <==
\section{Bayesian Credibility Region and Robust formulation}
\vspace{-1mm}
\label{section:Bayesian bounds and Robust formulation}

To estimate the system matrices $A_*, B_*$ after playing policy $\pi$ for $s$ steps, we use Regularized Least Squares estimator with regularizing parameter $\lambda$ defined as:
\begin{align}
\label{Regularized Least Squares Estimator}
    \widehat{A}, \widehat{B} = \argmin_{A, B}\sum_{i=0}^{s-1}\norm{x_{i+1}-Ax_i-Bu_i}_2 + \lambda \norm{(A~B)}_F.
\end{align}
In the following we will first show how we can obtain a credibility region $\Theta$ where the true system lies with high probability and then derive two controller synthesis procedures which result in a stabilizing controller for every system in region $\Theta$.

\subsection{Bayesian Credibility Region}
\label{subsection: Bayesian credibility Region}
\vspace{-1mm}
 To compute the credibility region $\Theta$ where system $A_*, B_*$ lies with high probability we follow the idea of \citet{Umenberer2019}. We a priori assume that the system matrices $A_*, B_*$ are sampled out of the Gaussian\footnote{Regarding the sense of this assumption and cases when this assumption fails look at \Cref{section: Data Dependent credibility Region}} distribution i.e. $\vectorized(A_*, B_*) \sim \pN\left(0, \frac{\sigma_w^2}{\lambda}I\right)$. In this case we have the explicit formulas for the posterior distribution of $\vectorized(A_*, B_*)|(x_j)_{j\le i}, (u_j)_{j<i}$. As derived in the \Cref{appendix: Posterior Distribution} it turns out that the MAP estimator is exactly the RLS estimator defined by \Cref{Regularized Least Squares Estimator}. Moreover, using the tail of $\chi_{d_x(d_x + d_u)}^2$ distribution, we define $\Theta= \{(A~B)|\Delta^\top D \Delta \preceq I, \Delta^\top = (A~B) - (\widehat{A}, \widehat{B})\}$. Here $D$ represents the scaled inverse covariance matrix of the posterior distribution and is explicitly given as $D = \frac{1}{c_\delta\sigma_w^2}\left(\sum_{j=1}^{i}z_jz_j^\top + \lambda I\right)$, where $z_j^\top = (x_j^\top u_j^\top)$ and $c_\delta$ is such that for $Z \sim \chi_{d_x(d_x + d_u)}^2$ we have $\pr(Z > c_\delta) = \delta$. With such a definition of $\Theta$ we have that $(A_*~B_*) \in \Theta$ w.p. $1-\delta$.

\subsection{Robust formulation from System Level Synthesis}
\label{subsection: Robust formulation from System Level Synthesis}
\vspace{-1mm}
In this section we will derive a procedure, using the SLS framework \citep{wang2019system}, which results in a controller $K$ which stabilizes all the systems is region $\Theta$ defined in \Cref{subsection: Bayesian credibility Region}. Assume that we have estimates $(\widehat{A}, \widehat{B})$. 
\citet{Dean2018OnSampleComplexity} show that controller $K$ stabilizes {\em all} systems $(A, B) \in \Theta$ if for every $(A~B) \in \Theta$ we have:
\begin{align}
\label{equation:HInfinityConditionToStabilize}
    \norm{
    \Delta^\top
    \begin{pmatrix}
     I \\
     K
    \end{pmatrix}
    \left(
    zI-\widehat{A}-\widehat{B}K
    \right)^{-1}
    }_{\mathcal{H}_\infty} < 1,
\end{align}
where $\Delta^\top = (A~B)-(\widehat{A}~\widehat{B})$. The $\mathcal{H}_\infty$-norm for a function $f: \C \to \C^{d \times d}$  is defined as $\norm{f}_{\mathcal{H}_\infty} = \sup_{z \in \partial \mathbb{D}}\norm{f(z)}$, where $\mathbb{D} = \{z\in \C|\norm{z}<1\}$ is a unit disk in the complex plane. To synthesize such a controller we first apply {\em S} lemma of \citet{LMIs2004} and obtain an equivalent problem with a single $\mathcal{H}_\infty$-norm constraint. We further transform the $\mathcal{H}_\infty$-norm constraint to convex semi-definite constraint by applying {\em KYP} \citep{KYPMoreReliableSource} lemma:
\begin{equation}
\label{semi-definite constraint}
    \begin{aligned}
    \text{Find } &X \succ 0, K, t \in (0, 1) \text{ with:} \\
    &\qquad\text{s.t.} 
     \begin{pmatrix}
    X - I & \widehat{A}X+\widehat{B}KX & 0  \\
    (\widehat{A}X+\widehat{B}KX)^\top & X & \begin{pmatrix} X \\ KX \end{pmatrix}^\top\\
    0 & \begin{pmatrix} X \\ KX \end{pmatrix} &tD \\
    \end{pmatrix}
    \succeq 0.
    \end{aligned}
\end{equation}
With the reparametrization $S=  KX$ the constraints given by \cref{semi-definite constraint} become convex.We show the details of the derivation that the existence of a controller $K$ satisfying \cref{equation:HInfinityConditionToStabilize} for every $(A~B) \in \Theta$ is equivalent to the feasibility of constraints in \cref{semi-definite constraint} in the \Cref{appendix: Semi Definite Program from SLS}. To find $X, S, t$ we propose to solve the following SDP: 
\begin{align}
\label{Convex SDP from SLS}
    \min_{X\succ 0, S, t\in (0, 1)}t \quad \text{s.t. } \cref{semi-definite constraint}    
\end{align}

\subsection{Robust formulation from Semi-Definite Program}
\label{subsection: Robust formulation from Semi-Definite Program}
\vspace{-1mm}
In the case when we know matrices $A_*, B_*$ we can obtain the the optimal controller $K_*$ by first solving the SDP
\begin{equation}
\label{optimal infinite hoizon policy SDP ineq}
\begin{aligned}
\min_{\Sigma \succeq 0}
    &\Tr\left(
    \begin{pmatrix}
        Q & 0 \\
        0 & R
    \end{pmatrix}
    \Sigma
    \right)\\
    &\text{s.t.} \quad
    \Sigma_{xx} \succeq (A_* ~ B_*)\Sigma (A_* ~ B_*)^\top  + \sigma_w^2 I,
\end{aligned}
\end{equation}
and then extracting the optimal controller as $K_* = \Sigma_{ux}\Sigma_{xx}^{-1}$. Here $\Sigma = \begin{pmatrix}\Sigma_{xx} & \Sigma_{xu} \\ \Sigma_{ux} & \Sigma_{uu}\end{pmatrix}$, where $\Sigma_{xx} \in \R^{d_x \times d_x}$ and $\Sigma_{uu} \in \R^{d_u \times d_u}$. The derivation with the motivation behind the SDP \eqref{optimal infinite hoizon policy SDP ineq} is given in \Cref{appendix: Optimal Infinite Horizon via SDP}. Using \Cref{lemma: Better covariance matrix for Epsilon region} we see that the semi-definite constraint in SDP \eqref{optimal infinite hoizon policy SDP ineq} ensures that controller synthesized as $K = \Sigma_{ux}\Sigma_{xx}^{-1}$ stabilize the system $A_*, B_*$. Inspired by this observation we pose the robust formulation of SDP \eqref{optimal infinite hoizon policy SDP ineq}:
\begin{equation}
\label{SDP: stabilizing SDP}
    \begin{aligned}
        \min_{\Sigma \succeq 0} &\Tr\left(
    \begin{pmatrix}
    Q & 0 \\
    0 & R
    \end{pmatrix}
    \Sigma
    \right)\\
    &\text{s.t. } \forall (A, B) \in \Theta: ~ 
    \Sigma_{xx} \succeq (A~B)\Sigma(A~B)^\top + \sigma_w^2 I.
    \end{aligned}
\end{equation}
As in \Cref{subsection: Robust formulation from System Level Synthesis} we have to ensure that one condition has to hold for every system in ellipsoid region $\Theta$. Applying S Lemma we reformulate problem given by \cref{SDP: stabilizing SDP} to an equivalent convex SDP:
\begin{equation}
\label{SDP: stabilizing SDP final}
    \begin{aligned}
        \min_{\Sigma \succeq 0, t \ge 0} &\Tr\left(
    \begin{pmatrix}
    Q & 0 \\
    0 & R
    \end{pmatrix}
    \Sigma
    \right)\\
    &\text{s.t. } 
    \begin{pmatrix}
        \Sigma_{xx} - (\widehat{A}~\widehat{B})\Sigma (\widehat{A}~\widehat{B})^\top - (t + \sigma_w^2) I & (\widehat{A}~\widehat{B})\Sigma \\
        \Sigma (\widehat{A}~\widehat{B})^\top & t D - \Sigma
    \end{pmatrix}\succeq 0.
    \end{aligned}
\end{equation}
The stabilizing controller is extracted from the optimal solution as $K = \Sigma_{ux}\Sigma_{xx}^{-1}$.

At first glance one could think that we have derived two completely different control synthesis procedures, however as we will see this is not the case.

\begin{theorem}
\label{theorem: feasibility equivalence}
    Robust SDP given by \Cref{Convex SDP from SLS} is feasible if and only if Robust SDP given by \Cref{SDP: stabilizing SDP final} is feasible.
\end{theorem}

The proof of the theorem is provided in \Cref{appendix: Proof of Theorem 1}. As we have seen in the \Cref{theorem: feasibility equivalence}, SDPs \eqref{Convex SDP from SLS} and \eqref{SDP: stabilizing SDP final} have feasible solutions at the same time. However, the minimization objectives are different, SDP \eqref{Convex SDP from SLS} is maximizing the ellipsoid region (instead of $D$ consider $\Theta$ associated with $tD$ with $t<1$) for which we can find a stabilizing controller
while SDP \eqref{SDP: stabilizing SDP final} is minimizing the upper bound of the maximal infinite horizon cost of the systems in $\Theta$.
